Adaptive Dynamic Programming for Energy-Efficient Base Station Cell Switching

Energy saving in wireless networks is growing in importance due to increasing demand for evolving new-gen cellular networks, environmental and regulatory concerns, and potential energy crises arising from geopolitical tensions. In this work, we propose an approximate dynamic programming (ADP)-based method coupled with online optimization to switch on/off the cells of base stations to reduce network power consumption while maintaining adequate Quality of Service (QoS) metrics. We use a multilayer perceptron (MLP) given each state-action pair to predict the power consumption to approximate the value function in ADP for selecting the action with optimal expected power saved. To save the largest possible power consumption without deteriorating QoS, we include another MLP to predict QoS and a long short-term memory (LSTM) for predicting handovers, incorporated into an online optimization algorithm producing an adaptive QoS threshold for filtering cell switching actions based on the overall QoS history. The performance of the method is evaluated using a practical network simulator with various real-world scenarios with dynamic traffic patterns.

==> background-related-works.tex <==
\section{Background and Related Work}\label{related-works}
%
Research related to our work is pertaining to base station switching (sleep mode management) techniques for energy saving. While these techniques will be addressed in the following in detail, many works concerning the energy saving problems using various methods in 4G wireless networks such as WiMAX and LTE, have shown promising results of energy saved \cite{salahdine2021survey, bousia2012energy}. 
%
Among those works, energy saving was formulated into optimization problems with certain perspective of the optimizable objects in addition to base station switching including improving the energy efficiency of the data transmission process \cite{li2014energy}, optimizing the distribution of the base stations \cite{coskun2014energy}, and utilizing renewable energy resources \cite{chia2014energy}, etc.
%
While in this work, we focus on the studies on base station switching, i.e., selectively switching off components with low occupation in base stations. 
%
Base station switching is considered to be an solution of being adaptable since its characteristics of fast adapting without requiring to change physical components of base stations \cite{wu2015energy}, feasible and applicable as base stations are designed to satisfy the peak traffic loads, the capacities are not always fully occupied \cite{feng2017base}.
%
% The challenges of the methods are the switching strategies for controlling the transmission delay made by overloaded traffic and increased handovers for the active base stations.
%

%
Base station switching methods concern mostly the network performance compromise such as delay and power consumption trad-eoff.
%
Some works consider a combined value of power consumption and delay to minimize either a weighted aggregation in order to have a flexible tradeoff \cite{son2011base}, or a minimal performance to power consumption ratio for reaching one time-step optimal \cite{tan2022graph}
%
Other works limit the performance compromise to be within a predetermined acceptable range but close to the allowed maximum to minimize the power consumption \cite{niu2015characterizing, salem2018reinforcement, salem2017advanced, ayala2018energy}.
%

%
In addition to the target trade-off,  various models were proposed and applied to find the optimal switching on/off solution based-on traffic condition and energy efficiency requirements.
%
Many rule-based models were proposed. Niu et al. \cite{niu2015characterizing} proposed a sleep mode strategy (named N-Policy) which put the base stations to sleep mode if no network access request from mobile users for a period of time.
%
Salem et al. \cite{salem2017advanced} performed base station switching between active and sleep modes periodically and maximized the sleep mode duration with the maximal delay tolerance for further energy saving.
%
Machine learning-based methods have been showing promising results in energy saving.
%
Pujol–Roigl et al. \cite{pujol2021deep} proposed a deep reinforcement learning method considering energy consumption, IP throughput rate, and handovers in the reward function.
%
Tan et al. \cite{tan2022graph} proposed a Graph Neural Network (GNN)-based methods for modeling the network topology into a graph where each base station is presented by a node embedding vector, which will eventually be mapped to a decision for switching on or off.
%
We intend to tackle the energy saving problem based on an Approximate Dynamic Programming (ADP) method, utilizing prior knowledge such as traffic patterns, Quality of Service (QoS) requirement patterns to have a control algorithm to solve large-scale optimization problem with feasibility and computational efficiency.
%
